Widespread Shocks in the Nucleus of NGC 404 Revealed by Near-infrared Integral Field Spectroscopy

We present high spatial resolution, integral field spectrograph (IFS) observations of the nearby LINER (low ionization nuclear emission line region) galaxy NGC 404 at 1.25 $\mu$m (J band) and 2.2 $\mu$m (K band) near-infrared wavelengths. Although NGC 404 is thought to host an intermediate mass black hole at its center, it has been unclear whether accretion onto the black hole or another mechanism such as shock excitation drives its LINER emission at optical/near-infrared wavelengths. We use the OSIRIS IFS at Keck Observatory behind laser guide star adaptive optics to map the strength and kinematics of [FeII], H$_2$, and hydrogen recombination lines at spatial resolutions of 1 pc across the central 30 pc of the galaxy. The H$_2$ gas is in a central rotating disk and ratios of multiple H$_2$ lines indicate that the molecular gas is thermally excited, with some contribution from UV fluorescence. The [FeII] emission is more extended and diffuse than the molecular gas and has a different kinematic structure that reaches higher velocities/dispersions. We also map the strength of the CO stellar absorption feature and constrain the dominant age of the nuclear stellar population to $\sim$1 Gyr. Finally, we find regions across the nucleus of NGC 404 with [FeII]/Pa$\beta$ line ratios up to 6.5, $\sim$2.5 times higher than the ratio measured from spatially-integrated spectra. From these high line ratios, we conclude that shocks are the dominate physical mechanism exciting NGC 404's LINER emission and argue that a possible source of this shock excitation is a supernova remnant.

==> line_ratio_results.tex <==
\begin{deluxetable*}{lrrrrrrrr}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{[FeII]/Pa$\beta$ and 1-0 S(1)/Br$\gamma$ Line Ratio Measurements in NGC 404}
\tablehead{
  \colhead{Aperture} & 
  \multicolumn{2}{c}{Aperture Location (arcsec)} & 
  \colhead{Radius} & 
  \multicolumn{2}{c}{Velocity Ranges (km sec$^{-1}$)\tablenotemark{b}} & 
  \colhead{[FeII]/} & 
  \colhead{1-0 S(1) H$_2$/} \\ 
% 
  \colhead{Number} & 
  \colhead{($\Delta$ RA)} & 
  \colhead{($\Delta$ DEC)} & 
  \colhead{(pixels)} & 
  \colhead{Line Flux} & 
  \colhead{Continuum\tablenotemark{b}} & 
  \colhead{Pa$\beta$\tablenotemark{c}} & 
  \colhead{Br$\gamma$\tablenotemark{c}} &
}
\startdata
\#1 & $0.00$ & $0.00$ & 4.0 & $\pm250$ & 300-450 & $-$ & $-$ \\ 
\#2 & $-0.22$ & $-0.28$ & 4.0 & $\pm200$ & 200-350 & $-$ & $-$ \\ 
\#3 & $-0.10$ & $-0.53$ & 4.0 & $\pm175$ & 175-325 & $4.3$ & $>2.6$ \\ 
\#4 & $0.00$ & $0.56$ & 4.0 & $\pm250$ & 300-450 & $5.7$ & $2.7$ \\ 
\#5 & $0.23$ & $0.49$ & 3.0 & $\pm250$ & 300-450 & $6.4$ & $>1.4$ \\ 
\#6 & $-0.09$ & $0.35$ & 2.0 & $\pm250$ & 300-450 & $6.0$ & $>1.1$ \\ 
\#7 & $0.09$ & $0.35$ & 2.5 & $\pm250$ & 300-450 & $5.3$ & $2.4$ \\ 
\#8 & $-0.16$ & $0.20$ & 3.0 & $\pm250$ & 300-450 & $6.5$ & $>2.8$ \\ 
\#9 & $0.02$ & $0.21$ & 2.0 & $\pm250$ & 300-450 & $2.5$ & $1.2$ \\ 
\#10 & $0.20$ & $0.20$ & 3.0 & $\pm175$ & 175-325 & $5.3$ & $>0.8$ \\ 
\#11 & $-0.26$ & $-0.02$ & 3.5 & $\pm250$ & 300-450 & $-$ & $-$ \\ 
\#12 & $0.26$ & $-0.04$ & 3.5 & $\pm250$ & 300-450 & $-$ & $-$ \\ 
\#13 & $0.06$ & $-0.28$ & 4.0 & $\pm250$ & 300-450 & $-$ & $-$ \\ 
\#14 & $0.29$ & $-0.34$ & 2.5 & $\pm200$ & 200-350 & $-$ & $-$ \\ 
\#15 & $0.18$ & $-0.55$ & 4.0 & $\pm175$ & 175-325 & $3.8$ & $>0.9$
\enddata 
\label{tab:lineratio_results}
\tablenotetext{a}{All velocity values are relative to the systemic velocity of the galaxy (-48 km sec$^{-1}$)}
\tablenotetext{b}{The velocity range given here refers to both the red (e.g., $+300$ - $+450$ km sec$^{-1}$) and blue (e.g., $-450$ - $-300$ km sec$^{-1}$) sides of the emission line.  Wavelength channels in these two ranges are used to estimate the continuum.}
\tablenotetext{c}{Line ratios measurements/upper limits are not reported for spectra with measured Pa$\beta$ absorption.}


\end{deluxetable*}

